Glissando-Net: Deep sinGLe vIew category level poSe eStimation ANd 3D recOnstruction

We present a deep learning model, dubbed Glissando-Net, to simultaneously estimate the pose and reconstruct the 3D shape of objects at the category level from a single RGB image. Previous works predominantly focused on either estimating poses(often at the instance level), or reconstructing shapes, but not both. Glissando-Net is composed of two auto-encoders that are jointly trained, one for RGB images and the other for point clouds. We embrace two key design choices in Glissando-Net to achieve a more accurate prediction of the 3D shape and pose of the object given a single RGB image as input. First, we augment the feature maps of the point cloud encoder and decoder with transformed feature maps from the image decoder, enabling effective 2D-3D interaction in both training and prediction. Second, we predict both the 3D shape and pose of the object in the decoder stage. This way, we better utilize the information in the 3D point clouds presented only in the training stage to train the network for more accurate prediction. We jointly train the two encoder-decoders for RGB and point cloud data to learn how to pass latent features to the point cloud decoder during inference. In testing, the encoder of the 3D point cloud is discarded. The design of Glissando-Net is inspired by codeSLAM. Unlike codeSLAM, which targets 3D reconstruction of scenes, we focus on pose estimation and shape reconstruction of objects, and directly predict the object pose and a pose invariant 3D reconstruction without the need of the code optimization step. Extensive experiments, involving both ablation studies and comparison with competing methods, demonstrate the efficacy of our proposed method, and compare favorably with the state-of-the-art.

==> response.tex <==
\subsection{Major Weakness 1}
We cited the suggested three papers \cite{fan2022object, langer2021leveraging, lee2021category} and added some text at the end of the second paragraph in Related Work. We compared with OLD-Net \cite{fan2022object} and NOCE \cite{lee2021category} on the NOCS dataset and reported the experimental results in Tables 1 and 3. We added the corresponding text in Sec 4.2. We also downloaded the code of Langer et al. \cite{langer2021leveraging} and tried to run their code. There are a lot of bugs in the code and the experimental results cannot be reproduced. We already emailed the authors and they provided the pretrained models and some missing files. But the code is still not executable. %download their pretrained models which are stored on google drive. But these pretrained models are expired. We already emailed the authors and we're still waiting for their response.
\subsection{Major Weakness 2}
We respectfully disagree with the reviewer's statement. First of all, we believe that the RGB information is learned successfully, by evidences from our ablation study in Table 7: we make Glissando-Net$_{DisEn}$ by disconnecting the feature transform module between RGB decoder and the point cloud encoder, and Glissando-Net$_{DisDe}$ by disconnecting the feature transform module between RGB decoder and the point cloud encoder (see Fig. \ref{fig:workflow}). Glissando-Net$_{DisEn}$ and Glissando-Net$_{DisDe}$ perform much worse than the original Glissando-Net on both shape reconstruction and pose estimation. 

Secondly, the reason we label the prediction of the red bottle in Figure 9 as a failure is mainly due to the special shape of that particular bottle as a long-tailed example in the bottle category. Specifically its shape resembles a cylindrical bottle and it is partially occluded. But if the RGB image input were, in fact, a partially occluded bottle, our prediction would have been categorically correct. We believe that if we include enough samples in the training data, we would be able to recover the correct shape of the specific bottle.

%All the examples in Figure 9 are failure cases for shape reconstruction. 
%Most results look good based on the quantitative results in Table 1. The first example (left column) shape is a long-tail example in the bottle category. Specifically its shape resembles a cylindrical bottle being partially occluded. Therefore, Glissando-Net successfully predicted the categorical shape.

%And the second and third examples are the shape reconstruction results of occluded RGB images which are generated by ourselves. They are not in the original training and testing set. RGB branch does a good job in providing the image feature to the 3D network based on Table 7. In Glissando-Net, RGB branch transfer 2D information through the transform module between RGB decoder and point cloud encoder\&decoder. In Table 7, we make Glissando-Net$_{DisEn}$ by disconnecting the feature transform module between RGB decoder and point cloud encoder, and Glissando-Net$_{DisDe}$ by disconnecting the feature transform module between RGB decoder and point cloud decoder (see Fig. \ref{fig:workflow}). Glissando-Net$_{DisEn}$ and Glissando-Net$_{DisDe}$ perform much worse than the original Glissando-Net on both shape reconstruction and pose estimation. 

\subsection{Major Weakness 3}
We projected the predicted point cloud with an estimated pose to the input on NOCS dataset. We added Figure \ref{fig:overlay} and added the corresponding text at the end of Sec 4.2.
\subsection{Minor Weakness 1}
During training, the point cloud encoder encodes the 3D shape, and the VAE forces the distribution of codes to be normal. In fact, the zero code during inference corresponds to the ‘mean’ shape of the training point clouds, similar to the usage in CodeSLAM ~\cite{bloesch2018codeslam}. For an ablation study, we removed the point cloud encoder, the feature transform module between the RGB decoder and point cloud encoder and the VAE bottleneck to create a baseline without the point cloud encoder. In this baseline, there is no code and the input is only the RGB image. In Tables 1, 2 and 3, the baseline without the point cloud encoder performs much worse than Glissando-Net in both 3D shape reconstruction and pose estimation, proving that our 3D encoder contributes significantly to both tasks.
\subsection{Minor Weakness 2}
We added the last row of result in Table 6 and added relevant text at the end of "Effects of the Pose Sub-network" in Sec. 4.4.
\subsection{Minor Weakness 3}
We added the last row of result in Table 8 and added some text at the end of the caption. We also added some text at the end of Sec. 4.5.
